Hierarchical Models for Relational Event Sequences

Interaction within small groups can often be represented as a sequence of events, where each event involves a sender and a recipient. Recent methods for modeling network data in continuous time model the rate at which individuals interact conditioned on the previous history of events as well as actor covariates. We present a hierarchical extension for modeling multiple such sequences, facilitating inferences about event-level dynamics and their variation across sequences. The hierarchical approach allows one to share information across sequences in a principled manner---we illustrate the efficacy of such sharing through a set of prediction experiments. After discussing methods for adequacy checking and model selection for this class of models, the method is illustrated with an analysis of high school classroom dynamics.

==> figures/dic-results.tex <==
% latex table generated in R 2.15.0 by xtable 1.7-0 package
% Wed Apr 25 17:03:00 2012
\begin{table}[ht]
\begin{center}
\begin{tabular}{lrrrr}
  \hline
 & A & B & C & F \\ 
  \hline
1 & 428258.68 & 435590.65 & 482480.37 & 484858.22 \\ 
  2 & 501634.92 & 540789.73 & 561368.16 & 562650.38 \\ 
  3 & 554216.93 & 599953.82 & 616154.27 & 616611.26 \\ 
   \hline
\end{tabular}
\caption{DIC under various model specifications for the hierarchical model fit to high school classroom interactions.  Lower is better.  Models with recency statistics tend to be preferred.}
\label{tab:classroom-dic}
\end{center}
\end{table}


==> figures/experiment-results.tex <==
% latex table generated in R 2.15.0 by xtable 1.7-0 package
% Mon Apr 30 00:35:40 2012
\begin{table}[ht]
\begin{center}
\begin{tabular}{rrp{2cm}p{2cm}}
  \hline
$z$ & $M_{train}$ & Mean recall imp. over $\hat{\mu}$ & Mean recall imp. over $\hat{\theta}^{ind}$ \\ 
  \hline
10 & 50 & 1.8 & 13.4 \\ 
   & 100 & 1.9 & 6.6 \\ 
   & 200 & 1.6 & 4.8 \\ 
  20 & 50 & 1.6 & 12.2 \\ 
   & 100 & 2.6 & 6.1 \\ 
   & 200 & 2.1 & 4.4 \\ 
  40 & 50 & 1.0 & 9.8 \\ 
   & 100 & 1.7 & 4.8 \\ 
   & 200 & 1.5 & 3.7 \\ 
   \hline
\end{tabular}
\caption{Prediction experiment on the classroom data.  Mean improvement in recall across classrooms for varying amounts of training data.}
\label{tab:classroom-recall}
\end{center}
\end{table}

